Extending Multilingual BERT to Low-Resource Languages

Multilingual BERT (M-BERT) has been a huge success in both supervised and zero-shot cross-lingual transfer learning. However, this success has focused only on the top 104 languages in Wikipedia that it was trained on. In this paper, we propose a simple but effective approach to extend M-BERT (E-BERT) so that it can benefit any new language, and show that our approach benefits languages that are already in M-BERT as well. We perform an extensive set of experiments with Named Entity Recognition (NER) on 27 languages, only 16 of which are in M-BERT, and show an average increase of about 6% F1 on languages that are already in M-BERT and 23% F1 increase on new languages.

==> 8-extra.tex <==

% our approach performs significantly better than \MBERT.
% Multilingual BERT (\MBERT) has achieved a huge success in transferring knowledge from high resource languages to low resource languages.
% Containing only the top 104 languages in Wikipedia, the official release of \MBERT does not address other languages (mainly low-resource languages) that it is never trained on.
% We propose a simple but effective way to extend the existing \MBERT to any language, with only a slight increase of additional training cost. 
% Our approach is to continue the pre-training process of \MBERT on the language of interest, thus allowing \MBERT to learn the new language.
% Through extensive experiments on several languages in Named Entity Recognition, we show that out method is able to ... 

% A natural way to apply the idea of Multilingual BERT to other languages is to train a new Multilingual BERT from scratch to include text data from target language, with the huge cost of training time.  In this paper, we propose an efficient approach to extend Multilingual BERT with a new language. With extensive experiments, we show that out approach is not only efficient, but also competitive(?) with Multilingual BERT trained from scratch.






==> tbl_stats.tex <==
\begin{table*}[!htbp]
\centering
\begin{tabular}{l 1 1 1 1 1 1 1 1 1 1 1 1 1 1 1 1 1 1 1} 
\toprule
\textbf{Lang} & Turkish	& Farsi	& Thai&	Bengali&Hungarian&	Russian	&Uzbek	&Tamil&	Indonesian	&Spanish&	Mandarin&	Hindi&	Tagalog&	Yoruba&	Swahili	&Arabic\\
\midrule
\bottomrule
\end{tabular}
\caption{}
\end{table*}

